Regularized Nonlinear Acceleration

We describe a convergence acceleration technique for unconstrained optimization problems. Our scheme computes estimates of the optimum from a nonlinear average of the iterates produced by any optimization method. The weights in this average are computed via a simple linear system, whose solution can be updated online. This acceleration scheme runs in parallel to the base algorithm, providing improved estimates of the solution on the fly, while the original optimization method is running. Numerical experiments are detailed on classical classification problems.

==> sections/ampe_old.tex <==
% !TEX root = ../reg_non_acc.tex
In what follows, we recall the key arguments behind {\em minimal polynomial extrapolation (MPE)} as derived in \citep{Caba76} or also \citep{Smit87}. We then explain a variant called {\em approximate minimal polynomial extrapolation (AMPE)} which allows to control the number of iterates used in the extrapolation, hence reduces its computational complexity. We begin by a simple description of the method for linear iterations, then extend these results to the generic nonlinear case. Finally, we characterize the acceleration factor provided by a regularized version of AMPE, using regularity properties of the function $f(x)$, and the result of a Chebyshev-like, tractable polynomial optimization problem.

\subsection{Linear Iterations}\label{ss:lin}
Let's assume for now that the iterative algorithm in~\eqref{eq:iter} is in fact linear, with
\BEQ\label{eq:iter-lin}
x_{i}=A (x_{i-1}-x^*) + x^*,
\EEQ
where $A\in\reals^{n \times n}$ (not necessarily symmetric) and $x^* \in \reals^n$. We assume that 1 is not an eigenvalue of $A$ (a sufficient condition is that the spectral radius of $A$ is below one, so the algorithm converges to $x^*$), implying that the iterations in~\eqref{eq:iter-lin} admits a unique fixed point $x^*$. 

\subsubsection*{Example: gradient method for minimizing a quadratic function}
We illustrate \eqref{eq:iter-lin} on a concrete example, minimizing the quadratic function $f(x) = \frac{1}{2}\|Bx-b\|_2^2$. The fixed-step gradient descend on $f(x)$ works as follows
\[
x_{k+1} = x_k-\frac{1}{L}\nabla f(x_k),
\]
where $f(x)$ is a $L$-smooth convex function. This scheme becomes here
\[
x_{k+1} = x_k - \frac{1}{L}(B^TBx_k/2-B^Tb)
\]
Using optimality conditions on $x^*$, this is also
\[
x_{k+1} = x_k - \frac{1}{L}B^TB(x_k-x^*)/2
\]
or again
\[
x_{k+1}-x^* = \left(I-\frac{1}{2L}B^TB\right)(x_k-x^*),
\]
which is exactly equation \eqref{eq:iter-lin} with $A = I-\frac{1}{2L}B^TB$.

\subsection{Minimal polynomial extrapolation}
We now recall the {\em minimal polynomial extrapolation} (MPE) method as described in~\citep{Smit87}, starting with the following definition. 

\begin{definition}\label{def:mpv}
	Given $A\in\reals^{n \times n}$, such that 1 is not an eigenvalue of $A$ and $v \in \reals^n$, the minimal polynomial of $A$ with respect to the vector $v$ is the lowest degree polynomial $p(x)$ such that
	\[
	p(A)v=0, \qquad p(1) = 1.
	\]
\end{definition}
Note that the degree of $p(x)$ is always less than $n$ and that condition $p(1)=1$ makes $p$ unique. Note also that assuming one is not an eigenvalue of $A$ means $p(1)\neq 0$, since $p(A)=0$ if and only if $p(\lambda_i(A))=0$ for $i=1,\ldots,n$, where $\lambda(A)$ is the spectrum of $A$. This means that we can set $p(1)=1$ without loss of generality. Given an initial iterate $x_0$, MPE starts by forming a matrix~$U$ whose columns are the increments $x_{i+1}-x_i $, with
\BEQ\label{eq:U-def}
U_{i}= x_{i+1}-x_i = (A-I)(x_i-x^*)=(A-I)A^i(x_0-x^*)=.
\EEQ
Let $p(x)=\sum_{i=0}^k c_i x^i$ be the minimal polynomial of $A$ with respect to the vector $U_0$, so
\BEQ
0= p(A)U_0=\sum_{i=0}^{k} c_iA^iU_0= \sum_{i=0}^{k} c_iU_i, \quad \mbox{and} \quad p(1) = \sum_{i=0}^{k} c_i = 1.
\label{eq:systemU}
\EEQ
Writing $U = [U_0,U_1,...,U_{k}]$, this means we can find the coefficients of~$p$ by solving the linear system
\[
Uc=0,~\ones^Tc=1.
\]
In this case, the fixed point $x^*$ of~\eqref{eq:iter-lin} can be computed {\em exactly} as follows. We have
\BEAS
0=\sum_{i=0}^{k} c_iA^iU_0  =  \sum_{i=0}^{k} c_i  A^i (A-I) (x_0-x^*) &=& (A-I) \sum_{i=0}^{k} c_i  A^i (x_0-x^*)\\
& = &  (A-I) \sum_{i=0}^{k} c_i  (x_i-x^*),
\EEAS
hence, using the fact that one is not an eigenvalue of $A$, together with $\ones^T c =p(1)=1$, we finally get
\[
x^* = \sum_{i=0}^{k} c_i  x_i. 
\]
This means that $x^*$ is obtained by {\em averaging} iterates using the coefficients in $c$, but the averaging is called nonlinear here because the coefficients of $c$ vary with the iterates themselves.



\subsection{Approximate Minimal Polynomial Extrapolation (AMPE)}\label{ss:ampe}
Suppose now that we only compute a fraction of the iterates $x_i$ used in the MPE procedure. While the number of iterates $k$ might be smaller than the degree of the minimal polynomial of $A$ with respect to $U_0$, we can still try to make the quantity $p_k(A)U_0$ small, with $p_k(x)$ now a polynomial of degree at most $k$. The corresponding difference matrix $U=[U_0,U_1,...,U_k]\in\reals^{n\times (k+1)}$ is rectangular. 

This is also known as the Eddy-Me{\v{s}}ina method \citep{Mesi77,Eddy79} or Reduced Rank Extrapolation with arbitrary $k$ (see \citep[\S10]{Smit87}). The objective here is similar to \eqref{eq:systemU}, but the system is now overdetermined because $k<\deg(P)$. We will thus choose $c$ to make $\|Uc\|_2=\|p(A)U_0\|_2$ as small as possible, for some polynomial $p$ such that $p(1)=1$. We thus solve for
\BEQ\label{eq:Rk}\tag{AMPE}
c^* \triangleq  \mathop{\mathrm{argmin}}\limits_{\ones^Tc=1} ~ \|Uc\|_2\\
\EEQ
in the variable $c\in\reals^{k+1}$. The optimal value of this problem is decreasing with $k$, satisfies $\|Uc^*\|_2=0$ when $k$ is greater than the degree of the minimal polynomial at $U_0$, and controls the approximation error in~$x^*$ through equation~\eqref{eq:U-def}. This basic extrapolation algorithm suffers from stability issues and we will see in further sections how to stabilize its solution.

\subsubsection{Error bounds}
We can get a crude bound on $\|Uc^*\|_2$ using Chebyshev polynomials, together with an assumption on the range of the spectrum of the matrix $A$. 

\begin{proposition} \label{prop:rateconvampe}
	Let $A$ be symmetric, $0\preceq A\preceq \sigma I$ with $\sigma<1$ and $c^*$ be the solution of \eqref{eq:Rk}. Then
	\BEA
	\label{eq:rateampe}
	\left\|\sum_{i=0}^k c^*_i x_i - x^*\right\|_2 \leq \kappa(A-I)\frac{2\zeta^k}{1+\zeta^{2k}}\|x_0-x^*\|_2
	\EEA
	where $\kappa(A-I)$ is the condition number of the matrix $A-I$ and $\zeta$ is given by
	\BEQ 
%	\label{eq:defzeta}
	\zeta = \frac{1-\sqrt{1-\sigma}}{1+\sqrt{1-\sigma}},
	\EEQ
	which is always smaller than $\sigma$.
\end{proposition}
\begin{proof} Setting $U_i=(A-I)(x_i-x^*)$, we have
	\BEAS
	\left\|\sum_{i=0}^k c^*_i x_i - x^*\right\|_2 & = & \left\|(I-A)^{-1} \sum_{i=0}^k c^*_i U_i\right\|_2\\
	& \leq & \left\|(I-A)^{-1}\right\|_2 \|Uc^*\|_2.
	\EEAS
	Assume $A$ symmetric and $0\preceq A \preceq \sigma I \prec I$, we have
	\BEA
	\|Uc^*\|_2  = \|p^*(A)U_0\|_2 \leq \|U_0\|_2 \min_{\substack{p\in\reals[x]\\p(1)=1}}\|p(A)\|_2 \leq \|U_0\|_2 \min_{\substack{p\in\reals[x]\\p(1)=1}}~\max_{0\preceq A \preceq \sigma I}\|p(A)\|_2.
	\label{eq:Ucstarcheby}
	\EEA
	We have $A = Q\diag(\lambda)Q^T$ where $Q$ is unitary and $\lambda\in\reals^n$, hence
	\[
	\max_{0\preceq A \preceq \sigma I}\|p(A)\|_2 =  \max_{0\preceq \lambda \preceq \sigma \ones}\|p(\diag(\lambda))\|_2 = \max_{0\preceq \lambda \preceq \sigma \ones} \max_i|p(\lambda_i)| = \max_{0\leq x\leq \sigma }|p(x)|.
	\]
	We then get
	\[
	\|Uc^*\|_2 \leq \|U_0\|_2\min_{\substack{p\in\reals[x]\\p(1)=1}}~\max_{0\leq x \leq \sigma}|p(x)|.
	\]
%	Now, \citet{Golu61} show that the polynomial optimization problem on the right-hand side can be solved exactly using Chebyshev polynomials. Let $C_k$ be the Chebyshev polynomial of degree $k$. By definition, $C_k(x)$ is a monic polynomial (i.e. a polynomial whose leading coefficient is one) which solves
%	\[ 
%	C_k(x) = \mathop{\mathrm{argmin}}\limits_{\{p\in\reals_k[x]:\, p_k=1\}} \;\max_{x\in[0,1]}|p(x)|.
%	\]
%	\citet{Golu61} use a variant of $C_k(x)$ to solve the related minimax problem
%	\BEQ\label{eq:chebyminimax}
%	\min_{\substack{p\in\reals[x]\\p(1)=1}}~\max_{0\leq x \leq \sigma}|p(x)|
%	\EEQ
%	whose solution is a rescaled Chebyshev polynomial given by 
%	\BEQ
%	T(x) = \frac{C_k(t(x))}{C_k(t(1))}, \quad \mbox{where}\quad t(x) =\frac{2x-\sigma}{\sigma},
%	\label{eq:rescaledcheby}
%	\EEQ
%	where $t(x)$ is simply a linear mapping from interval $[0,\sigma]$ to $[0,1]$. Moreover,
%	\BEQ\label{eq:chebysol}
%	\min_{\substack{p\in\reals[x]\\p(1)=1}}~\max_{0\leq x \leq \sigma}|p(x)| = \max_{0\leq x \leq \sigma}|T_k(x)| = |T_k(\sigma)| = \frac{2\zeta^k}{1+\zeta^{2k}},
%	\EEQ
%	where $\zeta$ is given by
%	\[
%	\zeta = \frac{1-\sqrt{1-\sigma}}{1+\sqrt{1-\sigma}} < \sigma <1.
%	\]
	Since $\|U_0\|_2 = \|(A-I)(x_0-x^*)\|_2 \leq \|A-I\|_2\|x_0-x^*\|$, we can bound \eqref{eq:Ucstarcheby} by
	\[
	\|Uc^*\|_2 \leq \|U_0\|_2\min_{\substack{p\in\reals[x]\\p(1)=1}}~\max_{0\leq x \leq \sigma}|p(x)| \leq \frac{2\zeta^k}{1+\zeta^{2k}}\|A-I\|_2\|x_0-x^*\|_2,
	\]
	which yields the desired result.
\end{proof}

Note that, when solving quadratic optimization problems (where gradient iterations are linear), the rate in this bound matches that obtained using the optimal method in \citep{Nest03a}. Outside of the normalization constraint, this is very similar to the convergence analysis of Lanczos' method.

\subsubsection{AMPE versus conjugate gradient} The rate of convergence obtained above also matches that of the conjugate gradient within a factor $\kappa(A-I)$. Indeed, AMPE has a strong link with the conjugate gradient. Denote $\|v\|_B = \sqrt{v^TBv}$ the norm induced by the positive definite matrix $B$. Also, assume we want to solve $Bx=b$ using conjugate gradient method. By definition, at the $k$-th iteration, the conjugate gradient computes an approximation $s$ of $x^*$ which follows
\[
s = \mathop{\mathrm{argmin}}\limits_{x \in \mathcal{K}_k} \|x-x^*\|_B,
\]
where $\mathcal{K}_k = \Span\{b,Bb,...,B^{k-1}b\} = \Span\{Bx^*,B^2x^*,...,B^{k}x^*\}$ is called a Krylov subspace. Since the constraint $x\in\mathcal{K}_k$ impose us to build $x$ from a linear combination of the basis of $\mathcal{K}_k$, we can write
\[
x = \sum_{i=1}^{k}c_iB^ix^* = q(B)x^*,
\] 
where $q(x)$ is a polynomial of degree $k$. So the  conjugate gradient method solves
\[ 
s = \mathop{\mathrm{argmin}}\limits_{\substack{q\in\reals_k[x]}\\q(0)=0} \|q(B)x^*-x^*\|_B  = \mathop{\mathrm{argmin}}\limits_{\substack{\hat q\in\reals_k[x]\\\hat q(0)=1}} \|\hat q(B)x^*\|_B,
\]
which is very similar to the equations in \eqref{eq:Rk}. However, while conjugate gradient has access to an oracle giving the result of the product between $B$ and any vector $v$, the AMPE procedure can only use the iterations produced by \eqref{eq:iter-lin} (meaning that AMPE procedure do not require knowledge of $B$). Moreover, the convergence of AMPE is analyzed in another norm ($\|\cdot\|_2$ instead of $\|\cdot\|_B$), which explains why a condition number appears in the rate of convergence of AMPE \eqref{eq:rateampe}.

\subsubsection{Chebyshev's acceleration and Nesterov's accelerated gradient} %\label{ss:cheby}
In proposition \ref{prop:rateconvampe}, we bounded the rate of convergence of the AMPE procedure using Chebyshev polynomials. In fact, this is exactly the idea behind Chebyshev's semi-iterative method, which uses these coefficients in order to accelerate gradient descent on quadratic functions. Here, we present Chebyshev semi-iterative acceleration and its analysis, then  use the same analysis on Nesterov's method. These points were also discussed in~\citep{Hard13}.

Assume as above that we use the gradient method to minimize $f(x)=\frac{1}{2}\|Bx-b\|_2$, we get the following recurrence
\[
x_{k+1}-x^* = \left(I-\frac{1}{L}B\right)(x_k-x^*) = A(x_k-x^*).
\]
Where $A = I-\frac{1}{L}B$. We see easily that 
\[
x_{k} = x^* + A^k(x_0-x^*).
\]
Since $\|A\|_2\leq 1-\frac{\mu}{L}$, the rate of convergence is $\|x_k-x^*\|_2 \leq (1-\frac{\mu}{L})^k\|x_0-x^*\|_2$. Moreover, if we combine linearly the vectors $x_i$ using coefficients $c_i$ from 0 to $k$, we get
\[
\sum_{i=0}^{k} c_ix_i = \sum_{i=0}^{k}c_iA^i(x_0-x^*) + \sum_{i=0}^{k}c_i x^* = p_k(A)(x_0-x^*)+p_k(1)x^*
\]
If we force $p_k(1) = 1$, we see that we need to make the value $\|p_k(A)(x_0-x^*)\|_2$ as small as possible in order to have the best approximation of $x^*$. Fixing the coefficients $c_i$ a priori (unlike AMPE method, which computes these coefficient from the iterates $x_i$) so that $\|p_k(A)\|_2$ is small for any $A$ such that $\mu I \preceq A\preceq L I$, means solving
\[
p_k(x) = \arg\min_{\substack{p\in\reals[x]\\p(1)=1}}~\max_{0\preceq A \preceq \sigma I}\left\|p\left(A\right)\right\|_2.
\]
As above, the solution to this problem is $p_k(x) = T_k(x)$, defined in~\eqref{eq:rescaledcheby}, using parameter $\sigma = 1-{\mu}/{L}$. Furthermore, the Chebyshev polynomials can be constructed using a three-terms recurrence
\[
C_k(x) = xC_{k-1}(x)-C_{k-2}(x)
\]
and the same holds for $T_k(x)$ (see Appendix \ref{app:chebyrecurence} for more details), with
\BEAS
\alpha_k &=& t(1)\alpha_{k-1}-\alpha_{k-2} \\
z_{k-1} &=& y_{k-1} - \frac{1}{L}(By_{k-1}-b) \\
y_{k} &=&  \frac{\alpha_{k-1}}{\alpha_{k}}\left(\frac{2z_{k-1}}{\sigma}-y_{k-1} \right)-\frac{\alpha_{k-2}}{\alpha_{k}}y_{k-2}
\EEAS
This scheme looks very similar to Nesterov's accelerated gradient method, which reads
\BEAS
z_{k-1} &=& y_{k-1} - \frac{1}{L}(By_{k-1}-b)\\
y_{k} &=& z_{k-1} + \beta_k(z_{k-1}-z_{k-2})
\EEAS
Compared with Chebyshev acceleration, Nesterov's scheme is iteratively building a polynomial $N_k(x)$ with $y_k-y^* = N_k\left(A\right)(y_0-x^*)$. If we replace $z_{k}$ by its definition in the expression of $y_k$ in the Nesterov's scheme we get the following recurrence of order two
\BEAS
y_{k}-x^* &=& (1+\beta_k)A(y_{k-1}-y^*) - \beta_k A(y_{k-2}-y^*)\\
&=& A\left((1+\beta_k)N_{k-1}\left(A\right) - \beta_k N_{k-2}\left(A\right)\right)(y_0-x^*).
\EEAS
which also reads
\[
N_k(x) = x((1+\beta_k)N_{k-1}(x) - \beta_k N_{k-2}(x)),
\] 
with initial conditions $N_0(x) = 1$ and $N_1(x) = x$. Notice that as for Chebyshev polynomial,  $N_k(1) = 1$ for all $k$. 

When minimizing smooth strongly convex functions with Nesterov's method, we use 
\[
\beta_k = \frac{\sqrt{L}-\sqrt{\mu}}{\sqrt{L}+\sqrt{\mu}}.
\] 
Moreover, empirically at least, the maximum value of $N_k(x)$ in the interval $[0,\sigma]$ is $N_k(\sigma)$. We conjecture that this always holds.
% AA: prove this
We thus have the following recurrence
\BEAS
N_{k}(\sigma) &=& \sigma\left(\left(1+\beta\right)N_{k-1}(\sigma) - \beta N_{k-2}(\sigma)\right)
\EEAS
To get linear convergence with rate $r$, we need $N_k\leq rN_{k-1} \leq r^2N_{k-2}$, or again
\[
N_{k}(\sigma) \leq \sigma\left(\left(1+\beta\right)rN_{k-2}(\sigma) - \beta N_{k-2}(\sigma)\right) =\sigma\left(\left(1+\beta\right)r - \beta \right) N_{k-2}(\sigma).
\]
Now, consider the condition
\[ 
\sigma\left(\left(1+\beta\right)r - \beta \right) \leq r^2.
\]
We have that Nesterov's coefficients and rate, i.e. $\beta={(1-\sqrt{\mu/L})}/{(1+\sqrt{\mu/L})}$ and $r = (1-\sqrt{\mu/L})$, satisfy this condition, showing that Nesterov's method converges with a rate at least $r=(1-\sqrt{\mu/L})$ on quadratic problems. This provides an alternate proof of Nesterov's acceleration result on these problemss using Chebyshev polynomials (provided the conjecture on $N(\sigma)$ holds).

\subsection{Nonlinear Iterations}\label{ss:nonlin}
We now go back to the general case where the iterative algorithm is nonlinear, with
\BEQ\label{eq:nonlinearalgo}
\tilde x_{i+1} = g( \tilde x_i), \quad \mbox{for $i=1,...,k$,}
\EEQ
where $\tilde x_i\in \reals^n$ and function $g(x)$ has a symmetric Jacobian at point $x^*$. We also assume that the method has a unique fixed point written $x^*$ and linearize these iterations around $x^*$, to get
\BEQ\label{eq:nonlin}
\rx_{i}-x^*=A(\rx_{i-1}-x^*) + e_{i},
\EEQ
where $A$ is now the Jacobian matrix (i.e. the first derivative) of $g$ taken at the fixed point $x^*$ and $e_i\in\reals^n$ is a second order error term $\|e_i\|_2=O(\|\tilde x_{i-1}-x^*\|_2^2)$. Note that, by construction, the linear and nonlinear models share the same fixed point~$x^*$. We write $x_i$ the iterates that would be obtained using the asymptotic linear model (starting at $x_0$)
\[
x_{i}-x^*=A (x_{i-1}-x^*).
\] 
After $k$ iterations, the accumulated error with respect to this asymptotic linear model is 
\[
\tilde x_k - x_k = \sum_{i=1}^k A^{k-i}e_i.
\]
As in \S\ref{ss:lin}, we define the increment matrix $U$ such that $U_{i}= x_{i+1}-x_{i}$ for $i=0,\ldots,k-1$, and a matrix $\tilde U$ constructed from $\rx$ in a similar way. Writing $E=\tilde U -U$ the corresponding error matrix, we have 
\[
E_{j+1}=\sum_{i=1}^{j+1} A^{j-i+1}e_i - \sum_{i=1}^j A^{j-i}e_i = (A-I)\left(\sum_{i=1}^j A^{j-i}e_i\right) + e_{j+1}, \quad j=0,\ldots,k-1.
\]
Assuming that $A$ is a contraction, i.e. that $\|A\|_2<1$, we can derive a crude bound on $\|E\|_2$ using the fact that
\[
\|E_{j+1}\|_2 \leq \|A-I\|_2 \sum_{i=1}^j \|A\|_2^{j-i}\|e_i\|_2 + \|e_{j+1}\|_2 \leq \frac{(1+\|I-A\|_2)\max_{i=1,\ldots,j+1} \|e_i\|_2}{1-\|A\|_2} ,
\]
which yields the following bound on the spectral norm of $E$
\BEQ\label{eq:E-bnd}
\|E\|_2 \leq \frac{\sqrt{k}~(1+\|I-A\|_2)\max_{i=1,\ldots,k} \|e_i\|_2}{1-\|A\|_2}.
\EEQ
%% FB: may be a better bound may be obtained by considering all columns of $E$ at once and using the fact that they share some parts?
Running the algorithm described in~\eqref{eq:nonlinearalgo}, we thus observe the iterates $\rx_i$ and build $\tilde U$ from their differences. As in~\eqref{eq:Rk} we then compute $\tilde c$ using matrix $\tilde U$ and finally estimate
\[
\rx^*= \sum_{i=0}^k \tilde c_j \rx_j.
\] 
In this case, our estimate for $x^*$ is based on the coefficient $\tilde c$, computed using the iterates $\tilde x_i$. The error induced in this estimate by the nonlinearity can be decomposed as
\BEQ \label{eq:boundampe}
\left\|\sum_{i=0}^k \tilde c_i \tilde x_i - x^*\right\|_2  \leq \left\|\sum_{i=0}^k (\tilde c_i-c_i) x_i \right\|_2 + \left\| \sum_{i=0}^k \tilde c_i  (\tilde x_i-x_i) \right\|_2 + \left\|\sum_{i=0}^k c_i x_i - x^* \right\|_2.
\EEQ
and we begin by showing the following proposition computing the perturbation $\Delta c = \tilde c^*-c^*$ of the optimal solution $c^*$ induced by~$E = \tilde U-U$, which will allow us to bound the first term on the right-hand side of~\eqref{eq:boundampe}.

\begin{proposition}\label{prop:stab}
	Let $c^*$ be the optimal solution to~\eqref{eq:Rk} 
	\[
	c^* = \mathop{\mathrm{argmin}}\limits_{\ones^Tc=1} ~ \|Uc\|_2\\
	\]
	for some matrix $U \in \reals^{n,k}$. Suppose $U$ becomes $\tilde U = U + E$, let $M = \tilde U^T\tilde U$ and write the perturbation matrix $P = \tilde U^T\tilde U - U^T U$, with $c^* + \Delta c$ the perturbed solution to~\eqref{eq:Rk}, then
	\BEQ \label{eq:delta-c}
	\Delta c = -\left(I - \frac{M^{-1}\ones\ones^T}{\ones^T M^{-1}\ones}\right)M^{-1}Pc^*
	\EEQ
	where
	\[
	\left(I - \frac{M^{-1}\ones\ones^T}{\ones^T M^{-1}\ones}\right)
	\]
	is a projector of rank $k-1$.
\end{proposition}
\begin{proof}
	Let $\mu$ be the dual variable corresponding to the equality constraint. Both $c^* + \Delta c$ and $\mu^* + \Delta \mu$ must satisfy the KKT system
	\BEAS
	\begin{bmatrix}
		2M & \ones \\ \ones^T & 0
	\end{bmatrix}
	\begin{pmatrix}
		c^* + \Delta c\\ \mu^*+\Delta \mu
	\end{pmatrix}
	= 
	\begin{pmatrix}
		0 \\ 1
	\end{pmatrix},
	\EEAS
	writing $P=U^TE+E^TU+E^TE$, this means again
	\BEAS
	\begin{bmatrix}
		2M & \ones \\ \ones^T & 0
	\end{bmatrix}
	\begin{pmatrix}
		c^* + \Delta c\\ \mu^*+\Delta \mu
	\end{pmatrix}
	&= 
	\begin{bmatrix}
		2P & 0 \\ 0 & 0
	\end{bmatrix}
	\begin{pmatrix}
		c^* + \Delta c\\ \mu^*+\Delta \mu
	\end{pmatrix}
	+
	\begin{bmatrix}
		2U^TU & \ones \\ \ones^T & 0
	\end{bmatrix}
	\begin{pmatrix}
		c^* + \Delta c\\ \mu^*+\Delta \mu
	\end{pmatrix}\\
	&= 
	\begin{pmatrix}
		2P (c^*+\Delta c) \\ 0
	\end{pmatrix}
	+
	\begin{bmatrix}
		2U^TU & \ones \\ \ones^T & 0
	\end{bmatrix}
	\begin{pmatrix}
		\Delta c\\ \Delta \mu
	\end{pmatrix}
	+
	\begin{pmatrix}
		0\\ 1
	\end{pmatrix}
	\EEAS
	hence
	\BEAS
	\begin{bmatrix}
		2M & \ones \\ \ones^T & 0
	\end{bmatrix}
	\begin{pmatrix}
		\Delta c\\ \Delta \mu
	\end{pmatrix}
	= \begin{pmatrix}
		-2Pc^* \\ 0
	\end{pmatrix}
	\EEAS
	The block matrix can be inverted explicitly, with
	\BEAS
	\begin{bmatrix}
		2M & \ones \\ \ones^T & 0
	\end{bmatrix}^{-1} = \frac{1}{\ones^T M^{-1} \ones}
	\begin{bmatrix}
		\frac{1}{2}M^{-1}\left((\ones^T M^{-1}\ones)I - \ones\ones^T M^{-1}\right) & M^{-1}\ones \\ \ones^T M^{-1} &-2
	\end{bmatrix}
	\EEAS
	leading to an expression of $\Delta c$ and $\Delta \mu$ in terms of $c^*$ and $\mu^*$:
	\BEAS
	\begin{pmatrix}
		\Delta c\\ \Delta \mu
	\end{pmatrix}
	= \frac{1}{\ones^T M^{-1} \ones}
	\begin{bmatrix}
		\frac{1}{2}M^{-1}\left((\ones^T M^{-1}\ones)I - \ones\ones^T M^{-1}\right) & M^{-1}\ones \\ \ones^T M^{-1} &-2
	\end{bmatrix}\begin{pmatrix}
		-2Pc^* \\ 0
	\end{pmatrix}
	\EEAS
	After some simplification, we get
	\BEAS
	\Delta c = -\left(I - \frac{M^{-1}\ones\ones^T}{\ones^T M^{-1}\ones}\right)M^{-1}Pc^* = -WM^{-1}Pc^*
	\EEAS
	where $W$ is a projector of rank $k-1$, which is the desired result.
\end{proof}
We see here that this perturbation can be arbitrarily large, which is the key issue with the convergence results in \citep[\S7]{Smit87}. Even if $\|c^*\|_2$ and $\|P\|_2$ are small, $M^{-1}$ is usually ill-conditioned. In fact, it can be shown that $U^TU$, which is the square of a Krylov matrix, has a condition number typically growing exponentially with the dimension \citep{Tyrt94}. Moreover, the eigenvalues are perturbed by $P$ which can make the situation even worse.
 


==> sections/error_bound_acc_grad.tex <==
% !TEX root = ../reg_non_acc.tex
Here, we fully explicit the bounds used in Section~\ref{ss:asympt} for the simple gradient method on smooth, strongly convex functions with Lipschitz-continuous Hessian. 

\subsection{Upper bound for $\|X-X^*\|_2$ and $\|U\|_2$}
Since we assumed that we used the gradient method, the sequence $\|\tilde x_k-x^*\|_2$ is monotone, following 
\[
\|\tilde x_{k+1}-x^*\| \leq r\|\tilde x_k-x^*\|
\]
In this case, we can bound easily $\|X-X^*\|_2$ with
\BEAS 
\|\tilde X-X^*\|_2 & \leq & \sum_{i=0}^k \|\tilde x_i-x^*\|_2 \\
& = & \frac{1-r^k}{1-r}\|x_0-x^*\|_2
\EEAS
Moreover, in the asymptotic model we have
\[
\|x_{k+1}-x^*\|_2 = \|A(x_{k}-x^*)\|_2 \leq \|A\|_2\|x_k-x^*\|_2
\]
where $A = I-\frac{1}{L}\nabla^2 f(x^*)$, so $\|A\|_2 \leq 1-\frac{L}{\mu}$. In that case,
\BEAS
\|U\|_2 & \leq & \|A-I\|_2 \sum_{i=0}^k \|x_i-x^*\|_2 \\
& \leq & \sum_{i=0}^k \|A\|^i \|x_0-x^*\|_2 \\
& \leq & \frac{1-\|A\|_2^k}{1-\|A\|_2}\|x_0-x^*\|_2 \\
& \leq & \frac{L}{\mu}\left(1-\left(1-\frac{\mu}{L}\right)^k\right)\|x_0-x^*\|_2
\EEAS

\subsection{Upper bound for $\|\mathcal{E}\|_2 = \|\tilde X-X\|_2$ and $\|E\|_2 = \|\tilde U-U\|$}
Since $\mathcal{E}_i = \tilde x_i-x_i$, we have
\[
\|\mathcal{E}\|_2 \leq \sum_{i=0}^k \|\tilde x_i-x_i\|_2
\]
%We will express $\|\tilde x_{i+1}-x_{i+1}\|_2$ in function of $\|\tilde x_0-x_0\|_2$ using a recursion with $\|\tilde x_i-x_i\|_2$:
%\BEAS\tilde x_{i+1} - x_{i+1} & = & \tilde x_i - \frac{1}{L}\nabla f(\tilde x_i) - x_i + \frac{1}{L} \nabla^2 f(x^*)(x_i-x^*)\\
%& = & \tilde x_{i} - x_{i} - \frac{1}{L}(\nabla f(\tilde x_i) - \nabla^2 f(x^*)(x_i-x^*)) \\
%& = & \left(I-\frac{\nabla^2 f(x^*)}{L}\right)(\tilde x_{i} - x_{i}) - \frac{1}{L}(\nabla f(\tilde x_i) - \nabla^2 f(x^*)(\tilde x_i-x^*)) 
%\EEAS
%Since our function has a Lipschitz-continuous Hessian, it is possible to show that (\cite{Nest03a}, \mbox{Lemma 1.2.4})
%\BEQ
%\left\|\nabla f(y) - \nabla f(x) - \nabla^2 f(x)(y-x)\right\|_2 \leq \frac{M}{2}\|y-x\|^2.
%\label{eq:boundhessianlipch}
%\EEQ
%We can thus bound the norm of the error at the $i^{\text{th}}$ iteration
%\BEAS
%\|x_{i+1}-\tilde x_{i+1}\|_2 & \leq & \left\| I-\frac{\nabla^2 f(x^*)}{L})\right\|_2 \| x_{i}-\tilde x_{i} \|_2 + \frac{1}{L}\left\|\nabla f(\tilde x_i) - \nabla^2 f(x^*)(\tilde x_i-x^*)\right\|_2\\
%& = & \left\| I-\frac{\nabla^2 f(x^*)}{L})\right\|_2\| x_{i}-\tilde x_{i} \|_2 + \frac{1}{L}\left\|\nabla f(\tilde x_i) - \nabla f(x^*) - \nabla^2 f(x^*)(\tilde x_i-x^*)\right\|_2\\
%\EEAS
%By equation \eqref{eq:boundhessianlipch}, we have
%\BEAS
%\|x_{i+1}-\tilde x_{i+1}\|_2 & \leq & (1-\frac{\mu}{L})\|  x_{i}-\tilde x_{i} \|_2 + \frac{M}{2L}\left\|\tilde x_i - x^*\right\|_2^2\\
%& \leq & (1-\frac{\mu}{L})\| x_{i}-\tilde x_{i}\|_2 + \frac{M}{2L}(r^2)^i \|x_0-x^*\|_2^2\\
%& = & \frac{M}{2L}\sum_{j=1}^{i}(1-\frac{\mu}{L})^{i-j}(r^2)^{j} \|x_0-x^*\|_2^2
%\EEAS
The sum starts at $j=1$ because, by definition, $\|e_0\|_2= \|\tilde x_0-x_0\|_2 = 0$. We can simplify this expression using the following property:
\BEQ
\frac{r^2}{1-\frac{\mu}{L}} = \frac{1}{1+\frac{\mu}{L}} < 1,
\label{eq:relationrkappa}
\EEQ
then bound $\|x_{i+1}-\tilde x_{i+1}\|_2$ as follows.
\BEAS 
\|x_{i+1}-\tilde x_{i+1}\|_2 &\leq & \left(1-\frac{\mu}{L}\right)^{i}\frac{M}{2L}\sum_{j=1}^{i}\left(\frac{r^2}{1-\frac{\mu}{L}}\right)^{j} \|x_0-x^*\|_2^2\\
&\leq & \left(1-\frac{\mu}{L}\right)^{i}\frac{M}{2L}\left(\sum_{j=0}^{i}\left(\frac{r^2}{1-\frac{\mu}{L}}\right)^{j}\right) \|x_0-x^*\|_2^2.
\EEAS
By equation \ref{eq:relationrkappa}, we can simplify the bound:
\[ 
\left(1-\frac{\mu}{L}\right)^{i}\frac{M}{2L}\left(\sum_{j=0}^{i}\left(\frac{r^2}{1-\frac{\mu}{L}}\right)^{j}\right) \|x_0-x^*\|_2^2 = \left(1-\frac{\mu}{L}\right)^{i}\frac{M}{2L}\left(\sum_{j=0}^{i}\left( \frac{1}{1+\frac{\mu}{L}}\right)^{j}\right) \|x_0-x^*\|_2^2
\]
We have thus
\BEAS
|x_{i+1}-\tilde x_{i+1}\|_2&\leq & \left(1-\frac{\mu}{L}\right)^{i}\frac{M}{2L}\left(\sum_{j=0}^{i}\left( \frac{1}{1+\frac{\mu}{L}}\right)^{j}\right) \|x_0-x^*\|_2^2\\ 
&=& \left(1-\frac{\mu}{L}\right)^{i}\frac{M}{2L}\left(\frac{1-\left(\frac{1}{1+\frac{\mu}{L}}\right)^i}{1-\frac{1}{1+\frac{\mu}{L}}}\right) \|x_0-x^*\|_2^2\\ 
&=& \frac{M}{2L}\left(\frac{(1-\frac{\mu}{L})^{i}-\left(\frac{1-\frac{\mu}{L}}{1+\frac{\mu}{L}}\right)^i}{1-\frac{1}{1+\frac{\mu}{L}}}\right) \|x_0-x^*\|_2^2\\ 
&=& \left(1+\frac{L}{\mu}\right)\frac{M}{2L}\left((1-\frac{\mu}{L})^{i}-\left(\frac{1-\frac{\mu}{L}}{1+\frac{\mu}{L}}\right)^i\right) \|x_0-x^*\|_2^2 .
\EEAS
By summing these error terms, we get
\BEAS
\|\mathcal{E}\|_2 & \leq & \sum_{i=0}^{k}\|x_{i}-\tilde x_{i}\|_2 \\
& \leq & \left(1+\frac{L}{\mu}\right)\frac{M}{2L}\left(\sum_{i=0}^{k}(1-\frac{\mu}{L})^{i}-\sum_{i=0}^{k}\left(\frac{1-\frac{\mu}{L}}{1+\frac{\mu}{L}}\right)^i\right) \|x_0-x^*\|_2^2\\ 
& = & \left(1+\frac{L}{\mu}\right)\frac{M}{2L}\left(\frac{L}{\mu}\left(1-\left(1-\frac{\mu}{L})^{k}\right)\right)-\frac{L}{2\mu}\left(1-\left(\frac{1-\frac{\mu}{L}}{1+\frac{\mu}{L}}\right)^k\right)\right) \|x_0-x^*\|_2^2\\ 
& \leq & \left(1+\frac{L}{\mu}\right)^2\frac{M}{2L}\left(1-\left(1-\frac{\mu}{L}\right)^{k}-\frac{1}{2}\left(1-\left(\frac{1-\frac{\mu}{L}}{1+\frac{\mu}{L}}\right)^k\right)\right) \|x_0-x^*\|_2^2\\ 
& = & \left(1+\frac{L}{\mu}\right)^2\frac{M}{2L}\left(\frac{1}{2}-\left(1-\frac{\mu}{L}\right)^{k}+\frac{1}{2}\left(\frac{1-\frac{\mu}{L}}{1+\frac{\mu}{L}}\right)^k\right) \|x_0-x^*\|_2^2
\EEAS
We finally have
\[ 
\|\tilde U - U\|_2 = \|E\|_2 \leq 2 \|\mathcal{E}\|_2 = \|\tilde X-X\|_2.
\]

\section{Two-terms recurence for Chebyshev's acceleration}
\label{app:chebyrecurence}
In this section we will details all steps to go from the theoretical definition of Chebyshev's acceleration
\[
y_k = T_k(A)(x_0-x^*)
\]
to the two-terms recurence
\BEAS
\alpha_k &=& t(1)\alpha_{k-1}-\alpha_{k-2} \\
z_{k-1} &=& y_{k-1} - \frac{1}{L}(Ay_{k-1}-b) \\
y_{k} &=&  \frac{\alpha_{k-1}}{\alpha_{k}}\left(\frac{2z_{k-1}}{\sigma}-y_{k-1} \right)-\frac{\alpha_{k-2}}{\alpha_{k}}y_{k-2}
\EEAS

Define $\alpha_k = C_k(t(1))$. Then, by definition of $T_k(x)$,
\[
\alpha_k T_k(x) = C_k(t(x))
\]
So, we get easily a three-term recurrence for $T_k(x)$
\BEAS
\alpha_k T_k(x) &=& C_k(t(x)) \\
&=& t(x)C_{k-1}(t(x))-C_{k-2}(t(x))\\ 
&=& t(x)\alpha_{k-1}T_{k-1}(x)-\alpha_{k-2}T_{k-2}(x)
\EEAS
and also for $\alpha_k$:
\BEAS
\alpha_k = C_k(t(1)) &=& t(1)\alpha_{k-1}C_{k-1}(t(1))-\alpha_{k-2}C_{k-2}(t(1))\\
&=& t(1)\alpha_{k-1}-\alpha_{k-2}
\EEAS
We will now see that we can form $y_k = \sum_{i=0}^k c_ix_i$ using only $y_{k-1}$ and $y_{k-2}$, where $x_k$ comes from the gradient method and $c_i$ are the coefficients of $T_k(x)$. We have
\BEAS
y_{k} -x^* &=& T_k\left(A\right)(x_0-x^*)\\
&=& \frac{1}{\alpha_{k}}\left(t\left(A\right)\alpha_{k-1}T_{k-1}(A)(x_0-x^*)-\alpha_{k-2}T_{k-2}(A)(x_0-x^*)\right)\\
&=& \frac{1}{\alpha_{k}}\left(\alpha_{k-1}t\left(A\right)(y_{k-1}-x^*)-\alpha_{k-2}(y_{k-2}-x^*)\right)\\
\EEAS
We need now to compute $t\left(A\right)y_{k-1}$. Since $t(x) = \frac{2x-\sigma}{\sigma}$, we have
\[
t\left(A\right)(y_{k-1}-x^*) = \frac{2\left(A\right)(y_{k-1}-x^*)-\sigma (y_{k-1}-x^*)}{\sigma}
\]
However, we have access to $x^*+A(y_{k-1}-x^*)$, since it correspond to a gradient step. Define 
\[
z_{k-1} = x^*+A(y_{k-1}-x^*) = y_{k-1} - \nabla f(y_{k-1})
\]
So,
\[
t\left(A\right)(y_{k-1}-x^*) = \frac{2(z_{k-1}-x^*)-\sigma (y_{k-1}-x^*)}{\sigma} = \frac{2z_{k-1}-\sigma y_{k-1}}{\sigma} - t(1)x^*
\]
If we plug this expression in the three-term recurrence,
\[
y_{k} -x^* = \frac{1}{\alpha_{k}}\left(\alpha_{k-1}\left(\frac{2z_{k-1}-\sigma y_{k-1}}{\sigma} - t(1)x^*\right)-\alpha_{k-2}(y_{k-2}-x^*)\right)
\]
Using the definition of $\alpha_k$, we can eliminate $x^*$ in both side. This leads to the following scheme.
\BEAS
z_{k-1} &=& y_{k-1} - \nabla f(y_{k-1}) \\
y_{k} &=&  \frac{\alpha_{k-1}}{\alpha_{k}}\left(\frac{2z_{k-1}}{\sigma}-y_{k-1} \right)-\frac{\alpha_{k-2}}{\alpha_{k}}y_{k-2}
\EEAS 

